Methods for Computing Legal Document Similarity: A Comparative Study

Computing similarity between two legal documents is an important and challenging task in the domain of Legal Information Retrieval. Finding similar legal documents has many applications in downstream tasks, including prior-case retrieval, recommendation of legal articles, and so on. Prior works have proposed two broad ways of measuring similarity between legal documents - analyzing the precedent citation network, and measuring similarity based on textual content similarity measures. But there has not been a comprehensive comparison of these existing methods on a common platform. In this paper, we perform the first systematic analysis of the existing methods. In addition, we explore two promising new similarity computation methods - one text-based and the other based on network embeddings, which have not been considered till now.

==> sections/relatedwork.tex <==
\section{Related Work}
\label{sec:related}
\vspace{-3mm}

Existing measures of similarity between legal documents can be broadly classified into network based and text based approaches. We describe methods from each approach next. \\
\textit{Network based Similarity measures: }
Existing network based similarity measures leverage prior-case judgments to build the network. A citation network of legal judgments is a directed graph, in which the vertices are the documents and a directed edge exists between vertices $v_i$ and $v_j$ if $v_i$ cites $v_j$.
The initial attempt at finding legal document similarity was in ~\cite{kumar2011similarity}. They used bibliographic coupling and co-citation to compute similarity between two documents. Dispersion was used in ~\cite{minocha2015finding} to compute similarity. Dispersion defines to what extent two individuals' mutual neighbours are not themselves well connected. An ontological approach using triple extraction was proposed in ~\cite{triplets}. They extract triplets using OpenIE and map the triplets to common terms and actors which have been identified by the legal domain ontology. They claim that similar documents will have a higher overlap in triplets.\\
\textit{Text based Similarity measures: }
Initial text based similarity measures were shown to work in ~\cite{kumar2011similarity}. Textual similarity between the paragraphs of legal documents and leveraging the idea of co-citation between the paragraphs was used to compute document similarity in ~\cite{kumar2013similarity}. A more recent study ~\cite{mandal2017measuring} has explored a wide range of legal document representation methods (eg., using whole document, a summary of the document, reason for citation of prior-judgments) and also state-of-the-art techniques (topic models, word embeddings and document embeddings) to calculate legal document similarity. They show that document embedding on the whole document have given the best result.
